Transferring Chemical and Energetic Knowledge Between Molecular Systems with Machine Learning

Predicting structural and energetic properties of a molecular system is one of the fundamental tasks in molecular simulations, and it has use cases in chemistry, biology, and medicine. In the past decade, the advent of machine learning algorithms has impacted on molecular simulations for various tasks, including property prediction of atomistic systems. In this paper, we propose a novel methodology for transferring knowledge obtained from simple molecular systems to a more complex one, possessing a significantly larger number of atoms and degrees of freedom. In particular, we focus on the classification of high and low free-energy states. Our approach relies on utilizing (i) a novel hypergraph representation of molecules, encoding all relevant information for characterizing the potential energy of a conformation, and (ii) novel message passing and pooling layers for processing and making predictions on such hypergraph-structured data. Despite the complexity of the problem, our results show a remarkable AUC of 0.92 for transfer learning from tri-alanine to the deca-alanine system. Moreover, we show that the very same transfer learning approach can be used to group, in an unsupervised way, various secondary structures of deca-alanine in clusters having similar free-energy values. Our study represents a proof of concept that reliable transfer learning models for molecular systems can be designed paving the way to unexplored routes in prediction of structural and energetic properties of biologically relevant systems.

==> images_old/Results_old.tex <==

\begin{figure}
    \centering
    \includegraphics[width=0.8\textwidth]{ROC.png}
    \caption{ROC Curve of model trained on alanine-dipeptide and tested on trialanine.}
    \label{fig:roc_curve}
\end{figure}

\begin{table}[]
    \centering
    \begin{tabular}{|c|c|c|c|c|c|}
    \hline
        Partition & RMSE & Correlation & Samples & Variance of data & Variance of prediction \\ \hline \hline
        Whole & 14.757397797860191 & 0.8193331292172209 & 100000 & 0.025814595062173824 & 0.025532173 \\ \hline
        Q1 & 9.478482463333572 & 0.24657727882605981 & 29927 & 0.0005686347557960356 & 0.0040573953 \\\hline
        Q2 & 12.394564207197849 & 0.31322625246779984 & 30965 & 0.00078136018471153 & 0.007427778 \\\hline
        Q3 & 13.506621062293148 & 0.5066194135741617 & 24635 & 0.002110246197897426 & 0.0107331285 \\\hline
        Q4 & 26.0723177339986 & 0.33465317181468823 & 14473 & 0.01938060511552492 & 0.017270828\\\hline
        Low & 8.112599984476093 & 0.045532224977848174 & 17378 & 0.00016076324680092553 & 0.0027932057 \\\hline
        High & 15.803294502030115 & 0.7838722977950383 & 82622 & 0.024317953732804282 & 0.024574324 \\\hline
    \end{tabular}
    \caption{Caption}
    \label{tab:errors}
\end{table}

\begin{table}[]
    \centering
    \begin{tabular}{|c|c|c|}
    \hline
         & Positive & Negative  \\ \hline \hline
        True & 13848 & 68847 \\\hline
        False & 3530 & 13775 \\\hline
    \end{tabular}
    \caption{Prec: 0.7968696052480148, Recall: 0.5013213626325888}
    \label{tab:prec}
\end{table}

\begin{figure}
    \centering
    \includegraphics[width=\textwidth]{sorted.png}
    \caption{Red: Actual Free Energy, Green: Predicted Free Energy}
    \label{fig:sorted}
\end{figure}
